Say More with Less: Understanding Prompt Learning Behaviors through Gist Compression

Large language models (LLMs) require lengthy prompts as the input context to produce output aligned with user intentions, a process that incurs extra costs during inference. In this paper, we propose the Gist COnditioned deCOding (Gist-COCO) model, introducing a novel method for compressing prompts which also can assist the prompt interpretation and engineering. Gist-COCO employs an encoder-decoder based language model and then incorporates an additional encoder as a plugin module to compress prompts with inputs using gist tokens. It finetunes the compression plugin module and uses the representations of gist tokens to emulate the raw prompts in the vanilla language model. By verbalizing the representations of gist tokens into gist prompts, the compression ability of Gist-COCO can be generalized to different LLMs with high compression rates. Our experiments demonstrate that Gist-COCO outperforms previous prompt compression models in both passage and instruction compression tasks. Further analysis on gist verbalization results suggests that our gist prompts serve different functions in aiding language models. They may directly provide potential answers, generate the chain-of-thought, or simply repeat the inputs. All data and codes are available at https://github.com/OpenMatch/Gist-COCO .

==> picture/embedding.tex <==
\begin{figure}[t]
    \centering
    \subfigure[Different Scenario.] { \label{fig:embed:compression} 
    \includegraphics[width=0.48\linewidth]{picture/image/three_compression_embedding.png}}
    \subfigure[Different Instruction.] { \label{fig:tasks} 
    \includegraphics[width=0.48\linewidth]{picture/image/three_task_embedding.png}}
    \caption{.}
    \label{fig:embed}
\end{figure}

==> picture/model_inference.tex <==

\begin{figure*}[ht]
\centering
\includegraphics[scale=0.65]{picture/image/Model_inference.png}
\caption{inference model.}
\label{fig:model}
\end{figure*}

==> picture/model_train.tex <==

\begin{figure*}[ht]
\centering
\includegraphics[scale=0.65]{picture/image/Model_train.png}
\caption{train model.}
\label{fig:model}
\end{figure*}

==> tables/average_token.tex <==
\begin{table}
\begin{center}
\small
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Model}&\textbf{Dataset} & \textbf{PopQA} & \textbf{KILT} & \textbf{Alpca+}  \\\hline
Average & 3.0   & 3.1  & 7.8   \\
Median  & 3.0   & 3.0  & 5.0    \\
\hline
\end{tabular}
\caption{Data Statistics of NOTICE model generation.}
\label{tab:token}
\end{center}
\end{table}

==> tables/different_passage.tex <==
\begin{table*}[t]
\small
\centering
\resizebox{\linewidth}{!}{
\scalebox{0.7}{
\begin{tabular}{l|l|c|ccc}
\hline
\multirow{2}{*}{\textbf{LLM}} & \multirow{2}{*}{\textbf{Model}}  & \multirow{2}{*}{\textbf{POPQA}}  & \multicolumn{3}{c}{\textbf{KILT}} \\
                                       &      &                          &  nq         & trivialqa         &    hotopqa                \\ \hline
\multirow{4}{*}{FlanT5-base}         
                                         & w / ours (1passage)                                 & 25.6         & 16.5       &  33.5      &    15.4        \\
                                            & w / ours (5passage)                                &  26.2       &  20.9      &  45.3      & 16.2          \\
                                      
                                        & w / 1passage                          & 34.8          & 22.9       &  46.7      & 20.0            \\ 
                                        & w / 5passage                          &  43.9        &  30.0      &   61.9     & 23.2       \\ \hline


\multirow{7}{*}{FlanT5-large}        
                                        & w / ours (1passage)                                 &  26.0       &  17.6    &   34.5  & 17.6             \\
                                        
                                        & w / ours (2passage)                                 &  29.1       & 20.0    &   43.6    & 18.4             \\

                                       & w / ours (5passage)                                 & 26.8        &  22.4     &   48.9  & 18.5          \\
                                      
                                        & w / 1passage                         &  34.6      &  25.3       &   51.1      & 23.8              \\ 

                                        & w / 2passage                         & 41.1         &   29.3     &   59.1     & 25.3            \\ 
                                        & w / 5passage                         &  46.0       &   34.4     &  67.1   & 27.5              \\ \hline

\multirow{7}{*}{Llama-7b}      & w / ours (1passage)                                & 31.0       & 24.3      &   64.0     &   21.5          \\


                                         & w / ours (2passage)                                &  32.0      & 25.2     &  65.8      &  21.8           \\

                                          & w / ours (5passage)                                & 30.1       &  25.8   &  66.0      &  20.8           \\
                                      
                                        & w / 1passage                          & 40.3         & 30.5     & 70.7       &   25.4          \\ 

                                         & w / 2passage                          &  43.5       &  32.4   &  73.1     &   25.8           \\ 
                                           & w / 5passage                          &   43.3      &  33.5   &  75.1     &  25.4            \\ \hline



\multirow{7}{*}{Llama-13b}                                         & w / ours  (1passage)                                 &  35.7    & 28.3        &       &               \\

                                        & w / ours  (2passage)                                 &  36.0   &         &       &               \\
                                         & w / ours  (5passage)                                 & 34.5     &   28.9    &       &               \\
                                      
                                        & w / 1passage                          & 41.8       &   31.1    &  73.8      & 28.3             \\ 

                                         & w / 2passage                          &    44.8   & 33.7     &  75.7      &  29.1            \\ 
                                         & w / 5passage                          &   45.7    &  36.0   &  77.6      &  29.3            \\ \hline


\multirow{7}{*}{Llama2-7b}                                          & w / ours (1passage)                                &   34.2       & 27.7      &        &               \\

                                         & w / ours (5passage)                                &  32.6      & 28.3      &        &              \\
                                      
                                        & w / 1passage                          & 40.5         & 29.9       &  72.5      &    27.3          \\ 
                                        & w / 2passage                          & 44.1         &  32.0      &  74.3      &   27.9           \\ 
                                        & w / 5passage                          &  45.2       & 35.0       &   75.4     &  27.9            \\ \hline
\end{tabular}
}}
\caption{Plug-In.}
\label{tab:diff_basemodel}
\end{table*}

==> tables/different_token.tex <==
\begin{table*}[t]

\centering
\resizebox{\linewidth}{!}{

\begin{tabular}{l|c|ccc|ccc}
\hline
\multirow{3}{*}{\textbf{Model}}  & \multicolumn{4}{c|}{\textbf{Passage Compression}} & \multicolumn{3}{c}{\textbf{Instruction Compression}} \\  \cline{2-8} & \multirow{2}{*}{\textbf{PopQA}}  & \multicolumn{3}{c}{\textbf{KILT}}  & \multicolumn{3}{c}{\textbf{Alpaca+}} \\\cline{3-8}  

                                                             &            &  NQ        & TrivialQA        & HotpotQA   &  Seen        & Unseen   &Human                   \\ \hline      

SEGENC &98.0\% &97.4\%	&97.3\%	&97.2\%		&32.7\%	&6.3\%	&50\% \\

Disentangled Gist-1 &99.5\%  &99.1\%	&99.2\%	&99.1\%		&43.6\%	&15.6\%	&35.2\%

    \\ 

Disentangled Gist-5 &99.5\% &99.1\%	&99.2\%	&99.1\%		&51.1\%	&22.9\%	&45.5\%
    \\ 

Disentangled Gist-10  &99.5\% &99.0\%	&99.2\%	&99.1\%		&49.8\%	&22.5\%	&43.5\%
  \\ 
  
                                        \hline



                                        

\end{tabular}}
\caption{Compression Ratio.}
\label{tab:diff_basemodel}
\end{table*}

==> tables/gist_data_analysis.tex <==
\begin{table*}[!ht]

\label{tab:case_study}
\small
\begin{tabular}{p{0.95\linewidth}}
\hline

\makecell{\textbf{Thinking Process}}
\tabularnewline 
\hline
\textbf{Original:} How would you go about finding the second largest element in an unsorted array? [-2, -1, 0, 1, 2]
\\

\textbf{Compression:} If 0 is the first element, then 0 is the second element.
\tabularnewline 
\\


\textbf{Original:} Explain what happens when we add or subtract fractions with unlike denominators.4/5 - 6/7
\\
\textbf{Compression:} The fractions are rounded to the nearest whole number.
\tabularnewline 
\hline

\makecell{\textbf{Repeat Query}}
\tabularnewline 
\hline
\textbf{Original:} Find a word in the dictionary whose letters are arranged alphabetically."zebra"
\\

\textbf{Compression:} zebra
\tabularnewline 
\\


\textbf{Original:} Write down a date on which you had an accident.Date: August 15, 2017
\\
\textbf{Compression:} August 15, 2017
\tabularnewline 
\hline


\makecell{\textbf{Given Answer}}
\tabularnewline 
\hline
\textbf{Original:} Do you think that the following sentences are true or false? justify your answers. Sentence: A square has four sides.
\\

\textbf{Compression:} yes
\tabularnewline 
\\


\textbf{Original:} Use these words in sentences.Word: "A"
\\
\textbf{Compression:} A is a word
\tabularnewline 
\hline

\makecell{\textbf{Other}}
\tabularnewline 
\hline
\textbf{Original:} Compute the longest increasing subsequence from a sorted list of integers.[2, 3, 4, 5, 6]'
\\

\textbf{Compression:} 1, 3, 5, 6, 7, 8, 9, 10, 11, 13, 14, 15, 16, 17, 19, 20, 21, 22, 23
\tabularnewline 
\hline
\end{tabular}
\caption{instruction}
\end{table*}


==> tables/overall_new.tex <==
\begin{table*}[t]

\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|l|c|ccc|ccc}
\hline
\multirow{3}{*}{\textbf{LLM}} & \multicolumn{1}{l|}{\multirow{3}{*}{\textbf{Model}}}  & \multicolumn{4}{c|}{\textbf{Passage Compression}} & \multicolumn{3}{c}{\textbf{Instruction Compression}} \\  \cline{3-9}   &   & \multirow{2}{*}{\textbf{PopQA}}  & \multicolumn{3}{c}{\textbf{KILT}}  & \multicolumn{3}{c}{\textbf{Alpaca+}} \\\cline{4-9}  

                                            &                        &            &  NQ        & TrivialQA        & HotpotQA   &  Seen        & Unseen   &Human                   \\ \hline
\multirow{7}{*}{FlanT5-base}          & zero-shot                                                   & 8.8         &  4.4       &  9.2        & 12.1    &  20.3        &  22.0     &  9.7                    \\
                                       & w / AutoCompressor                      &  8.3        &   4.8     &   9.4      &   12.2  &20.3 & 22.7 & 7.8          \\
                                       & w / Gist                               &    8.4      &  4.6        & 8.9    & 12.1     &18.3  &18.9 &  8.7        \\
                                
                                            & w / ours                                &        &22.9        &        &    &        &        &        \\
                                      
                    
                                        & w / context                           &  43.9        &  30.0      &   61.9     & 23.2   &  23.9      &   29.8     &  15.2     \\ \hline


\multirow{7}{*}{FlanT5-large}          & zero-shot                                                   &  7.3        & 8.3       &  19.0        &     14.6  & 19.2     &  18.4       &  10.3              \\
                                       & w / AutoCompressor                       &   5.8       &  8.4      &    19.1     &  14.7  &16.6   & 12.2 &  6.6           \\
                                       & w / Gist                               &    9.1     &  8.2          &  18.9      & 14.6    & 21.4 &19.0 &  10.7        \\

                                        & w / Gist(ours) &11.3&7.3&17.5&13.4&24.3&28.7&15.9 \\
                                    
                                        & w / ours  &27.4 &23.7 &52.4 &19.3 &25.0  &28.8  &14.0   \\
                                        & w / context                          &  46.0       &   34.4     &  67.1   & 27.5    &  26.7      &  32.3      &   18.8                 \\ \hline



\end{tabular}
}
\caption{Plug-In. Compression 5 passages}
\label{tab:diff_basemodel}
\end{table*}

==> tables/passage_analysis.tex <==
\begin{table*}[t]
\label{tab:case_study}
\small
\scalebox{0.95}{
\begin{tabular}{p{0.95\linewidth}}
\hline

\makecell[c]{\textbf{POPQA Dataset}}
\tabularnewline 
\hline
\textbf{Passage:} The Economics and Ethics of Private Property
 The Economics and Ethics of Private Property: Studies in Political Economy and Philosophy (1993; second edition 2006) is a book about private property by the economist \textcolor[HTML]{FA8072}{Hans-Hermann Hoppe}.
 Section::::Publishing history ....
\\
\textbf{Query:} Q: Who is the author of The Economics and Ethics of Private Property? A:.
\\
\tabularnewline 
\textbf{Compression:} \textcolor[HTML]{FA8072}{Hans-Hermann Hoppe}
\tabularnewline 
\hline

\makecell[c]{\textbf{NQ Dataset}}
\tabularnewline 
\hline
\textbf{Passage:} "Photograph" is a song by English musician Ringo Starr that was released as the lead single from his 1973 album "Ringo". Starr co-wrote the song with \textcolor[HTML]{FA8072}{George Harrison}, his former bandmate from the Beatles. Although the two of them collaborated on other compositions, it is the only song officially credited to the pair...
\\
\textbf{Query:} who wrote the song photograph by ringo start
\\
\tabularnewline 
\textbf{Compression:}  \textcolor[HTML]{FA8072}{George Harrison}
\tabularnewline 
\hline


\makecell[c]{\textbf{TriviaQA Dataset}}
\tabularnewline 
\hline
\textbf{Passage:} "Up Where We Belong" is a song written by Jack Nitzsche, Buffy Sainte-Marie and Will Jennings that was recorded by Joe Cocker and Jennifer Warnes for the 1982 film  \textcolor[HTML]{FA8072}{"An Officer and a Gentleman"}. Warnes was recommended to sing a song from the film because of her previous soundtrack successes...
\\
\textbf{Query:} who wrote the song photograph by ringo start
\\
\tabularnewline 
\textbf{Compression:}  \textcolor[HTML]{FA8072}{An Officer and a Gentleman}
\tabularnewline 
\hline

\makecell[c]{\textbf{HotpotQA Dataset}}
\tabularnewline 
\hline
\textbf{Passage:} The Vermont Catamounts men's soccer team represents the University of Vermont in all NCAA Division I men's college soccer competitions. The team competes in the \textcolor[HTML]{FA8072}{America East Conference}.
\\
\textbf{Query:} The Vermont Catamounts men's soccer team currently competes in a conference that was formerly known as what from 1988 to 1996?
\\
\tabularnewline 
\textbf{Compression:}  \textcolor[HTML]{FA8072}{America East Conference}
\hline
\end{tabular}
}
\caption{instruction}
\end{table*}


==> tables/verblize.tex <==
\begin{table*}[t]
\small
\centering
\resizebox{\linewidth}{!}{
\scalebox{0.95}{
\begin{tabular}{l|l|c|ccc|ccc}
\hline
\multirow{3}{*}{\textbf{LLM}} & \multirow{3}{*}{\textbf{Model}}& \multicolumn{4}{c|}{\textbf{Passage Compression}}& \multicolumn{3}{c}{\textbf{Instruction Compression}} \\  \cline{3-9}

& & \multirow{2}{*}{\textbf{PopQA}}  & \multicolumn{3}{c|}{\textbf{KILT}} & \multicolumn{3}{c}{\textbf{Alpaca+}}\\ \cline{4-9}
                                            &                        &             &  NQ        & TrivialQA        & HotpotQA   & Seen & Unseen   &Human               \\ \hline




\multirow{4}{*}{Llama-7b}          & zero-shot                                                   & 22.8         &  20.5       &  61.7        &    18.2   & 21.7  	&  21.1 & 4.6           \\

                                       & w / SEGENC                                   &  25.3        &  23.9      &   62.5    &  19.3   &  25.6	 & 25.0	 & 8.1
      \\


    

                                           & w / ours (large)                             &31.2 &26.8 &68.5 &22.2 &24.6	&25.1	&8.6
\\

                                           & w / context                          &   43.3      &  33.5   &  75.1     &  25.4   &36.0	 &34.4	 &12.5
         \\ \hline

\multirow{4}{*}{Llama2-7b-hf}          & zero-shot                                                   &  26.0       & 24.0        &    67.8      &     20.9 &21.3 &20.8 &6.2		                \\
                                        & w / SEGENC                                 &  28.6       &  27.4      &   69.0    &  20.8  &26.1	&24.7	&8.6
         \\





                                          & w / ours (large)                           &32.7 &29.4 &71.2 &23.9 &21.7	&24.1	&7.6

                                         \\
                                      
                                        & w / context                         &  45.2       & 35.0       &   75.4     &  27.9 &35.5	&32.8	&12.3
     \\ \hline


\multirow{4}{*}{Llama-13b}          & zero-shot                                                   & 27.6         &  27.2       &  72.9        &   22.0  &22.3 &  18.7  &4.0              \\
                                
                                        & w / SEGENC                                 &  31.2      & 29.7      & 70.6      &   22.3 &27.7	&26.2	&9.5
          \\

                                        & w / ours (large)                                 & 34.0     &29.3  &74.0 & 24.0 &24.7	&25.3	&9.5
     \\
                                         
                                      
                                         & w / context                           &   45.7    &  36.0   &  77.6      &  29.3     & 37.6	& 38.0	& 14.4
   \\ \hline


                                    

\end{tabular}
}}
\caption{Generalize to other models.}
\label{tab:diff_basemodel}
\end{table*}
